Nonwatertight Mesh Reconstruction

Reconstructing 3D non-watertight mesh from an unoriented point cloud is an unexplored area in computer vision and computer graphics. In this project, we tried to tackle this problem by extending the learning-based watertight mesh reconstruction pipeline presented in the paper 'Shape as Points'. The core of our approach is to cast the problem as a semantic segmentation problem that identifies the region in the 3D volume where the mesh surface lies and extracts the surfaces from the detected regions. Our approach achieves compelling results compared to the baseline techniques.

==> tbl/table1-clean.tex <==
\begin{center}
\begin{longtable}{|m{0.31\textwidth}| m{0.31\textwidth} | m{0.31\textwidth}|}
\hline
{\bfseries Pipeline} &
\raggedleft{\bfseries Chamfer Distance ($\downarrow$)} &
\raggedleft\arraybslash{\bfseries Hausdorff Distance ($\downarrow$)}\\\hline\hline
SAP &
\raggedleft 0.009798 &
\raggedleft\arraybslash 0.254690\\\hline
SAP(freezed) + SMPN &
\raggedleft 0.000615 &
\raggedleft\arraybslash 0.108691\\\hline
\cellcolor{SpringGreen!50}SAP + SMPN &
\cellcolor{SpringGreen!50} \raggedleft{\bfseries 0.000239} &
\cellcolor{SpringGreen!50} \raggedleft\arraybslash{\bfseries 0.071070}\\\hline
\caption{Quantitative comparison of the performances of the extended pipeline (2nd and 3rd row) with the base pipline (1st row) on the ShapeNet dataset (mean over 5 classes).}
\label{table1}
\end{longtable}
\end{center}


==> tbl/table1.tex <==
\begin{center}
\begin{longtable}{|m{0.31\textwidth}| m{0.31\textwidth} | m{0.31\textwidth}|}
\hline
{\bfseries Pipeline} &
\raggedleft{\bfseries Chamfer Distance ($\da$)} &
\raggedleft\arraybslash{\bfseries Hausdorff Distance ($\da$)}\\\hline\hline
SAP &
\raggedleft 0.009798 &
\raggedleft\arraybslash 0.254690\\\hline
SAP(freezed) + SMPN &
\raggedleft 0.000615 &
\raggedleft\arraybslash 0.108691\\\hline
\cellcolor{SpringGreen!50}SAP + SMPN &
\cellcolor{SpringGreen!50} \raggedleft{\bfseries 0.000239} &
\cellcolor{SpringGreen!50} \raggedleft\arraybslash{\bfseries 0.071070}\\\hline
\caption{Quantitative comparison of the performances of the extended pipeline (2nd and 3rd row) with the base pipline (1st row) on the ShapeNet dataset (mean over 5 classes).}
\label{table1}
\end{longtable}
\end{center}


==> tbl/table2-clean.tex <==
\begin{center}
\begin{longtable}{m{0.05\textwidth}|m{0.2125\textwidth}|m{0.2125\textwidth}|m{0.2375\textwidth}|m{0.2125\textwidth}}
~
 &
\centering Input &
\centering SAP &
\centering SAP Extended &
\centering\arraybslash GT Mesh\\\hline &&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/sn1.png} &
\includegraphics[width=\linewidth]{img/table1/sn1sap.png} &
\includegraphics[width=\linewidth]{img/table1/sn1p.png} &
\includegraphics[width=\linewidth]{img/table1/1g.png}\\&&&&\\
\centering \rotatebox[origin=c]{90}{Low Noise} &
\includegraphics[width=\linewidth]{img/table1/sn2.png} &
\includegraphics[width=\linewidth]{img/table1/sn2sap.png} &
\includegraphics[width=\linewidth]{img/table1/sn2p.png} &
\includegraphics[width=\linewidth]{img/table1/2g.png}\\&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/sn3.png} &
\includegraphics[width=\linewidth]{img/table1/sn3sap.png} &
\includegraphics[width=\linewidth]{img/table1/sn3p.png} &
\includegraphics[width=\linewidth]{img/table1/3g.png}\\\hline &&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/ln1.png} &
\includegraphics[width=\linewidth]{img/table1/ln1sap.png} &
\includegraphics[width=\linewidth]{img/table1/ln1p.png} &
\includegraphics[width=\linewidth]{img/table1/1g.png}\\&&&&\\
\centering \rotatebox[origin=c]{90}{High Noise} &
\includegraphics[width=\linewidth]{img/table1/ln2.png} &
\includegraphics[width=\linewidth]{img/table1/ln2sap.png} &
\includegraphics[width=\linewidth]{img/table1/ln2p.png} &
\includegraphics[width=\linewidth]{img/table1/2g.png}\\&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/ln3.png} &
\includegraphics[width=\linewidth]{img/table1/ln3sap.png} &
\includegraphics[width=\linewidth]{img/table1/ln3p.png} &
\includegraphics[width=\linewidth]{img/table1/3g.png}\\\hline&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/o1.png} &
\includegraphics[width=\linewidth]{img/table1/o1sap.png} &
\includegraphics[width=\linewidth]{img/table1/o1p.png} &
\includegraphics[width=\linewidth]{img/table1/1g.png}\\&&&&\\
\centering \rotatebox[origin=c]{90}{Outliers} &
\includegraphics[width=\linewidth]{img/table1/o2.png} &
\includegraphics[width=\linewidth]{img/table1/o2sap.png} &
\includegraphics[width=\linewidth]{img/table1/o2p.png} &
\includegraphics[width=\linewidth]{img/table1/2g.png}\\&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/o3.png} &
\includegraphics[width=\linewidth]{img/table1/o3sap.png} &
\includegraphics[width=\linewidth]{img/table1/o3p.png} &
\includegraphics[width=\linewidth]{img/table1/3g.png}\\&&&&\\
\caption{Qualitative comparison of the performances of the extended pipeline with the base pipline in 3 different types of input.}
\label{table2}
\end{longtable}
\end{center}


==> tbl/table2.tex <==
\begin{center}
\begin{longtable}{m{0.05\textwidth}|m{0.2125\textwidth}|m{0.2125\textwidth}|m{0.2375\textwidth}|m{0.2125\textwidth}}
~
 &
\centering Input &
\centering SAP &
\centering SAP Extended &
\centering\arraybslash GT Mesh\\\hline &&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/sn1.png} &
\includegraphics[width=\linewidth]{img/table1/sn1sap.png} &
\includegraphics[width=\linewidth]{img/table1/sn1p.png} &
\includegraphics[width=\linewidth]{img/table1/1g.png}\\&&&&\\
\centering \rotatebox[origin=c]{90}{Low Noise} &
\includegraphics[width=\linewidth]{img/table1/sn2.png} &
\includegraphics[width=\linewidth]{img/table1/sn2sap.png} &
\includegraphics[width=\linewidth]{img/table1/sn2p.png} &
\includegraphics[width=\linewidth]{img/table1/2g.png}\\&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/sn3.png} &
\includegraphics[width=\linewidth]{img/table1/sn3sap.png} &
\includegraphics[width=\linewidth]{img/table1/sn3p.png} &
\includegraphics[width=\linewidth]{img/table1/3g.png}\\\hline &&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/ln1.png} &
\includegraphics[width=\linewidth]{img/table1/ln1sap.png} &
\includegraphics[width=\linewidth]{img/table1/ln1p.png} &
\includegraphics[width=\linewidth]{img/table1/1g.png}\\&&&&\\
\centering \rotatebox[origin=c]{90}{High Noise} &
\includegraphics[width=\linewidth]{img/table1/ln2.png} &
\includegraphics[width=\linewidth]{img/table1/ln2sap.png} &
\includegraphics[width=\linewidth]{img/table1/ln2p.png} &
\includegraphics[width=\linewidth]{img/table1/2g.png}\\&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/ln3.png} &
\includegraphics[width=\linewidth]{img/table1/ln3sap.png} &
\includegraphics[width=\linewidth]{img/table1/ln3p.png} &
\includegraphics[width=\linewidth]{img/table1/3g.png}\\\hline&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/o1.png} &
\includegraphics[width=\linewidth]{img/table1/o1sap.png} &
\includegraphics[width=\linewidth]{img/table1/o1p.png} &
\includegraphics[width=\linewidth]{img/table1/1g.png}\\&&&&\\
\centering \rotatebox[origin=c]{90}{Outliers} &
\includegraphics[width=\linewidth]{img/table1/o2.png} &
\includegraphics[width=\linewidth]{img/table1/o2sap.png} &
\includegraphics[width=\linewidth]{img/table1/o2p.png} &
\includegraphics[width=\linewidth]{img/table1/2g.png}\\&&&&\\
~
 &
\includegraphics[width=\linewidth]{img/table1/o3.png} &
\includegraphics[width=\linewidth]{img/table1/o3sap.png} &
\includegraphics[width=\linewidth]{img/table1/o3p.png} &
\includegraphics[width=\linewidth]{img/table1/3g.png}\\&&&&\\
\caption{Qualitative comparison of the performances of the extended pipeline with the base pipline in 3 different types of input.}
\label{table2}
\end{longtable}
\end{center}


==> tbl/table3-clean.tex <==
\begin{table}[H]
\begin{longtable}{|m{0.20\textwidth}|m{0.14\textwidth}|m{0.29\textwidth}|m{0.29\textwidth}|}
\hline
{\bfseries Method} &
\raggedleft{\bfseries Threshold} &
\raggedleft{\bfseries Chamfer Distance ($\downarrow$)}&
\raggedleft\arraybslash{\bfseries Hausdorff Distance ($\downarrow$)}\\\hline\hline
2D Laplacian &
\raggedleft 0.00 &
\raggedleft 0.009798 &
\raggedleft\arraybslash 0.254690\\\hhline{~---}
~
 &
\raggedleft {\bfseries 0.05} &
\raggedleft {\bfseries 0.008534} &
\raggedleft\arraybslash {\bfseries 0.254473}\\\hhline{~---}
~
 &
\raggedleft 0.10 &
\raggedleft 0.009470 &
\raggedleft\arraybslash 0.254429\\\hhline{~---}
~
 &
\raggedleft 0.20 &
\raggedleft 0.016016 &
\raggedleft\arraybslash 0.260365\\\hhline{~---}
~
 &
\raggedleft 0.40 &
\raggedleft 0.059645 &
\raggedleft\arraybslash 0.340960\\\hhline{----}
3D Laplacian &
\raggedleft 0.00 &
\raggedleft 0.009799 &
\raggedleft\arraybslash 0.254690\\\hhline{~---}
~
 &
\raggedleft {\bfseries 0.05} &
\raggedleft {\bfseries 0.008783} &
\raggedleft\arraybslash {\bfseries 0.254579}\\\hhline{~---}
~
 &
\raggedleft 0.10 &
\raggedleft 0.010009 &
\raggedleft\arraybslash 0.254576\\\hhline{~---}
~
 &
\raggedleft 0.20 &
\raggedleft 0.023703 &
\raggedleft\arraybslash 0.255712\\\hhline{~---}
~
 &
\raggedleft 0.40 &
\raggedleft 0.088625 &
\raggedleft\arraybslash 0.400718\\\hhline{----}\hline
\cellcolor{SpringGreen!50}Ours &
\cellcolor{SpringGreen!50} \raggedleft {}- &
\cellcolor{SpringGreen!50} \raggedleft{\bfseries 0.000239} &
\cellcolor{SpringGreen!50} \raggedleft\arraybslash{\bfseries 0.071070}\\\hline
\caption{Quantitative comparison of the performances of the extended pipeline with the baseline methods on the ShapeNet dataset (mean over 5 classes). The table shows performances of the kernel methods (2D/3D Laplacian) for mask generation at various thresholds.}
\label{table3}
\end{longtable}
\end{table}

==> tbl/table3.tex <==
\begin{table}[H]
\begin{longtable}{|m{0.20\textwidth}|m{0.14\textwidth}|m{0.29\textwidth}|m{0.29\textwidth}|}
\hline
{\bfseries Method} &
\raggedleft{\bfseries Threshold} &
\raggedleft{\bfseries Chamfer Distance ($\da$)}&
\raggedleft\arraybslash{\bfseries Hausdorff Distance ($\da$)}\\\hline\hline
2D Laplacian &
\raggedleft 0.00 &
\raggedleft 0.009798 &
\raggedleft\arraybslash 0.254690\\\hhline{~---}
~
 &
\raggedleft {\bfseries 0.05} &
\raggedleft {\bfseries 0.008534} &
\raggedleft\arraybslash {\bfseries 0.254473}\\\hhline{~---}
~
 &
\raggedleft 0.10 &
\raggedleft 0.009470 &
\raggedleft\arraybslash 0.254429\\\hhline{~---}
~
 &
\raggedleft 0.20 &
\raggedleft 0.016016 &
\raggedleft\arraybslash 0.260365\\\hhline{~---}
~
 &
\raggedleft 0.40 &
\raggedleft 0.059645 &
\raggedleft\arraybslash 0.340960\\\hhline{----}
3D Laplacian &
\raggedleft 0.00 &
\raggedleft 0.009799 &
\raggedleft\arraybslash 0.254690\\\hhline{~---}
~
 &
\raggedleft {\bfseries 0.05} &
\raggedleft {\bfseries 0.008783} &
\raggedleft\arraybslash {\bfseries 0.254579}\\\hhline{~---}
~
 &
\raggedleft 0.10 &
\raggedleft 0.010009 &
\raggedleft\arraybslash 0.254576\\\hhline{~---}
~
 &
\raggedleft 0.20 &
\raggedleft 0.023703 &
\raggedleft\arraybslash 0.255712\\\hhline{~---}
~
 &
\raggedleft 0.40 &
\raggedleft 0.088625 &
\raggedleft\arraybslash 0.400718\\\hhline{----}\hline
\cellcolor{SpringGreen!50}Ours &
\cellcolor{SpringGreen!50} \raggedleft {}- &
\cellcolor{SpringGreen!50} \raggedleft{\bfseries 0.000239} &
\cellcolor{SpringGreen!50} \raggedleft\arraybslash{\bfseries 0.071070}\\\hline
\caption{Quantitative comparison of the performances of the extended pipeline with the baseline methods on the ShapeNet dataset (mean over 5 classes). The table shows performances of the kernel methods (2D/3D Laplacian) for mask generation at various thresholds.}
\label{table3}
\end{longtable}
\end{table}

==> tbl/table4-clean.tex <==
\begin{table}[p]
\begin{longtable}{m{0.18\linewidth}|m{0.18\linewidth}|m{0.18\linewidth}|m{0.18\linewidth}|m{0.18\linewidth}}
\centering Input &
{\centering 2D Laplacian\par}

\centering (with best threshold) &
{\centering 3D Laplacian\par}

\centering (with best threshold) &
\centering SAP Extended &
\centering\arraybslash Ground Truth\\\hline\hline &&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/1.png} &
\centering \includegraphics[width=\linewidth]{img/table2/12d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/13d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/1p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/1g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/2.png} &
\centering \includegraphics[width=\linewidth]{img/table2/22d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/23d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/2p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/2g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/3.png} &
\centering \includegraphics[width=\linewidth]{img/table2/32d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/33d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/3p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/3g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/4.png} &
\centering \includegraphics[width=\linewidth]{img/table2/42d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/43d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/4p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/4g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/5.png} &
\centering \includegraphics[width=\linewidth]{img/table2/52d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/53d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/5p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/5g.png}\\
\caption{Qualitative comparison of the performances of the extended pipeline with the baseline methods (with the best threshold for mask generation) on the ShapeNet dataset.}
\label{table4}
\end{longtable}
\end{table}


==> tbl/table4.tex <==
\begin{table}[p]
\begin{longtable}{m{0.18\linewidth}|m{0.18\linewidth}|m{0.18\linewidth}|m{0.18\linewidth}|m{0.18\linewidth}}
\centering Input &
{\centering 2D Laplacian\par}

\centering (with best threshold) &
{\centering 3D Laplacian\par}

\centering (with best threshold) &
\centering SAP Extended &
\centering\arraybslash Ground Truth\\\hline\hline &&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/1.png} &
\centering \includegraphics[width=\linewidth]{img/table2/12d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/13d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/1p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/1g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/2.png} &
\centering \includegraphics[width=\linewidth]{img/table2/22d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/23d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/2p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/2g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/3.png} &
\centering \includegraphics[width=\linewidth]{img/table2/32d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/33d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/3p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/3g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/4.png} &
\centering \includegraphics[width=\linewidth]{img/table2/42d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/43d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/4p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/4g.png}\\&&&&\\
\centering \includegraphics[width=\linewidth]{img/table2/5.png} &
\centering \includegraphics[width=\linewidth]{img/table2/52d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/53d.png} &
\centering \includegraphics[width=\linewidth]{img/table2/5p.png} &
\centering\arraybslash \includegraphics[width=\linewidth]{img/table2/5g.png}\\
\caption{Qualitative comparison of the performances of the extended pipeline with the baseline methods (with the best threshold for mask generation) on the ShapeNet dataset.}
\label{table4}
\end{longtable}
\end{table}


==> tbl/table5-clean.tex <==
\begin{table}[H]
\begin{longtable}{|l|r|r|r|r|}
\hline
\diagbox{Metric}{Kernel Width} &
\raggedleft 3 &
\raggedleft 5 &
\raggedleft 7 &
\raggedleft\arraybslash 9\\\hline
Chamfer Distance &
0.000172
 &
\textbf{0.000174}
 &
0.000221
 &
0.000263
\\\hline
Hausdorff Distance &
0.047733
 &
\textbf{0.042084}
 &
0.060259
 &
0.058211
\\\hline
\caption{Ablation study over kernel width}
\label{table5}
\end{longtable}
\end{table}

==> tbl/table5.tex <==
\begin{table}[H]
\begin{longtable}{|l|r|r|r|r|}
\hline
\diagbox{Metric}{Kernel Width} &
\raggedleft 3 &
\raggedleft 5 &
\raggedleft 7 &
\raggedleft\arraybslash 9\\\hline
Chamfer Distance &
0.000172
 &
\bf{0.000174}
 &
0.000221
 &
0.000263
\\\hline
Hausdorff Distance &
0.047733
 &
\bf{0.042084}
 &
0.060259
 &
0.058211
\\\hline
\caption{Ablation study over kernel width}
\label{table5}
\end{longtable}
\end{table}

==> tbl/tablez.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lllll}
5                     & 6                     &                       &                       &                       \\ \cline{2-5} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cline{2-5} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cline{2-5} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cline{2-5} 
\end{tabular}
\caption{This is a table}
\label{table1}
\end{table}

m{0.33\textwidth}
\bottomcaption{some caption}
\label{table1}
